A benchmark of categorical encoders for binary classification

Categorical encoders transform categorical features into numerical representations that are indispensable for a wide range of machine learning models. Existing encoder benchmark studies lack generalizability because of their limited choice of (1) encoders, (2) experimental factors, and (3) datasets. Additionally, inconsistencies arise from the adoption of varying aggregation strategies. This paper is the most comprehensive benchmark of categorical encoders to date, including an extensive evaluation of 32 configurations of encoders from diverse families, with 36 combinations of experimental factors, and on 50 datasets. The study shows the profound influence of dataset selection, experimental factors, and aggregation strategies on the benchmark's conclusions -- aspects disregarded in previous encoder benchmarks.

==> notes.tex <==
% Parts to change 29.11.22 - updated 13.03.23

0. The focus should shift from "benchmark to find the best" to "experiment to determine the effect of factors", which allows me to focus more on those and rankings rather than encoders themselves. It is also a necessary addition to the existing literature.
00. Journal: IEEE TKDE should be a good fit
T. Conclusions: deeper studies are required even in a simple topic as encoders. This means that the current studies are not enough. We found that some encoders overall work better than others, 
X. we are using a relaxed version of HK rank as we constrain only for transitivity and totality
Z1. citations for datasets 
Z2. inconsistent notation for adjacency matrices. Use $M^l$
Z3. add citations for RAS in experiment:consensus
Z4. add to RAS discussion that our ranks are obtained just by average. Why? because t-test ranking CANNOT ensure transitivity
Z5. could be worth showing why we wnt transitivity and totality for a ranking
Z6. should a rank start from 0 or 1? 0 is more natural in calculations, 1 is more natural for a humna. is it?
Z7. Use consistent capitalization for $\Phi$ scoring function
Z8. leftover rank aggregation: best $n$. left out because we have ranks with different cardinalities. Maybe based on threshold?
Z9. in experiment:consensus:rescaled mean score, the minimum and maximum symbols are not great
ZA. \%nans in the dataset table is actually a fraction. 
ZB. Add fundamentals section and put details of encoders and RAS in there
ZC. related work: current sota comparisons + takeaway shortcomings
ZD. Tuning times are unstable - due to repeated experiments, I know that some runs are very slower than others for no apparent reason
ZE. Add citation to openML as from https://openml.github.io/openml-python/main/
ZF. Add a simple example table for encoding
ZG. Move encoder abbreviations to experimental design. Possibly change them
ZH. Encoder Abkurzungen are not consistent in formulas they appear as math objects
ZI. Pseudocode for PreBinnedEncoder in Appendix
ZJ. Add \noindent to subsections and paragraphs (as from https://www.jmlr.org/format/format.html)'
ZK. For the new rank similarity measure: 1. check existing literature on sensitivity analysis + kemeny aggregation + papers citing the 1998 one proposing weight tau
ZL. Motivate tau b over rho (RAS literature)
ZM. weighted taub: use simple weights, such as: linear decreasing. Compare constant weights against tau b. 
ZN. plots with HUE for different sim metrics (shows everything) 







% Characteristics from Bengio's "Representation Learning: A Review and New Perspectives"
1. "The advantages are A and B." then proceeds with dedicated paragraphs
2. 


==> sections/Y_checklist.tex <==
\section*{Checklist}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Section~\ref{sec:results}.}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:conclusions}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{Our research might bring better experimental comparisons of encoders, but will likely not affect the broader society.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We provide them in Appendix~\ref{sec:appendix:experiments}, as well as a link to our code in the Abstract.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Appendix~\ref{sec:appendix:experiments}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Section~\ref{sec:results}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix~\ref{sec:appendix:results}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{In the published code.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{In the published code.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{We limit our study to open-source datasets.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> tables/datasets_complete.tex <==

% datasets
\begin{table*}[htb]
\caption{Datasets used in the analysis.} 
\centering
\label{tab:datasets}
\begin{tabular}{lcccccccc}
\toprule
\textbf{name} & \textbf{ID} & \textbf{obs} & \textbf{feats} & \textbf{bins} & \textbf{cats} & \textbf{nums} & \textbf{\%nans} & \textbf{mostclasses} \\ \midrule
\emph{kr-vs-kp} & 3 & 3196 & 36 & 35 & 1 & 0 & 0.0 & 3 \\
\emph{credit-approval} & 29 & 690 & 15 & 3 & 6 & 6 & 0.0 & 15 \\
\emph{credit-g} & 31 & 1000 & 20 & 3 & 11 & 7 & 0.0 & 10 \\
\emph{sick} & 38 & 3772 & 29 & 19 & 2 & 6 & 0.1 & 5 \\
\emph{tic-tac-toe} & 50 & 958 & 9 & 0 & 9 & 0 & 0.0 & 3 \\
heart-h & 51 & 294 & 13 & 2 & 6 & 6 & 0.2 & 4 \\
\emph{vote} & 56 & 435 & 16 & 0 & 16 & 0 & 0.1 & 3 \\
\emph{monks-problems-1} & 333 & 556 & 6 & 2 & 4 & 0 & 0.0 & 4 \\
\emph{monks-problems-2} & 334 & 601 & 6 & 2 & 4 & 0 & 0.0 & 4 \\
\emph{irish} & 451 & 500 & 5 & 1 & 2 & 2 & 0.0 & 11 \\
\emph{profb} & 470 & 672 & 9 & 1 & 3 & 5 & 0.2 & 28 \\
\emph{mv} & 881 & 40768 & 10 & 2 & 1 & 7 & 0.0 & 3 \\
\emph{molecular-biology\_promoters} & 956 & 106 & 57 & 1 & 56 & 0 & 0.0 & 4 \\
nursery & 959 & 12960 & 8 & 1 & 7 & 0 & 0.0 & 5 \\
\emph{kdd\_internet\_usage} & 981 & 10108 & 68 & 48 & 20 & 0 & 0.0 & 129 \\
\emph{ada\_prior} & 1037 & 4562 & 14 & 1 & 7 & 6 & 0.0 & 40 \\
KDDCup09\_appetency & 1111 & 50000 & 230 & 6 & 33 & 174 & 0.7 & 15416 \\
KDDCup09\_churn & 1112 & 50000 & 230 & 6 & 33 & 174 & 0.7 & 15416 \\
KDDCup09\_upselling & 1114 & 50000 & 230 & 6 & 33 & 174 & 0.7 & 15416 \\
airlines & 1169 & 539383 & 7 & 0 & 4 & 3 & 0.0 & 293 \\
Agrawal1 & 1235 & 1000000 & 9 & 0 & 3 & 6 & 0.0 & 20 \\
bank-marketing & 1461 & 45211 & 16 & 3 & 6 & 7 & 0.0 & 12 \\
\emph{blogger} & 1463 & 100 & 5 & 2 & 3 & 0 & 0.0 & 5 \\
nomao & 1486 & 34465 & 118 & 2 & 27 & 89 & 0.0 & 3 \\
\emph{thoracic-surgery} & 1506 & 470 & 16 & 10 & 3 & 3 & 0.0 & 7 \\
\emph{wholesale-customers} & 1511 & 440 & 8 & 0 & 1 & 7 & 0.0 & 3 \\
\emph{adult} & 1590 & 48842 & 14 & 1 & 7 & 6 & 0.0 & 42 \\
amazon\_employee\_access & 4135 & 32769 & 9 & 0 & 9 & 0 & 0.0 & 7518 \\
\emph{cylinder-bands} & 6332 & 540 & 37 & 0 & 17 & 18 & 0.1 & 71 \\
\emph{dresses-sales} & 23381 & 500 & 12 & 0 & 11 & 1 & 0.1 & 25 \\
\emph{SpeedDating} & 40536 & 8378 & 120 & 3 & 58 & 59 & 0.0 & 260 \\
Titanic & 40945 & 1309 & 13 & 1 & 6 & 6 & 0.2 & 1307 \\
\emph{Australian} & 40981 & 690 & 14 & 4 & 4 & 6 & 0.0 & 14 \\
\emph{jungle\_chess\_2pcs\_endgame\_elephant\_elephant} & 40999 & 2351 & 46 & 19 & 2 & 20 & 0.0 & 3 \\
\emph{jungle\_chess\_2pcs\_endgame\_rat\_rat} & 41005 & 3660 & 46 & 21 & 2 & 20 & 0.0 & 3 \\
\emph{jungle\_chess\_2pcs\_endgame\_lion\_lion} & 41007 & 2352 & 46 & 21 & 2 & 20 & 0.0 & 3 \\
kick & 41162 & 72983 & 32 & 1 & 17 & 14 & 0.0 & 1063 \\
porto-seguro & 41224 & 595212 & 57 & 18 & 13 & 26 & 0.0 & 104 \\
telco-customer-churn & 42178 & 7043 & 19 & 6 & 11 & 3 & 0.0 & 6531 \\
KDD98 & 42343 & 82318 & 477 & 29 & 107 & 341 & 0.1 & 18543 \\
sf-police-incidents & 42344 & 538638 & 6 & 0 & 5 & 1 & 0.0 & 21838 \\
open\_payments & 42738 & 73558 & 5 & 1 & 4 & 0 & 0.2 & 4374 \\
Census-Income-KDD & 42750 & 199523 & 41 & 2 & 27 & 13 & 0.1 & 51 \\
\emph{students\_scores} & 43098 & 1000 & 7 & 2 & 2 & 3 & 0.0 & 6 \\
WMO-Hurricane-Survival-Dataset & 43607 & 5021 & 22 & 0 & 21 & 1 & 0.0 & 4173 \\
law-school-admission-bianry & 43890 & 20800 & 11 & 4 & 1 & 6 & 0.0 & 6 \\
\emph{national-longitudinal-survey-binary} & 43892 & 4908 & 16 & 4 & 4 & 9 & 0.0 & 29 \\
\emph{ibm-employee-attrition} & 43896 & 1470 & 34 & 3 & 5 & 26 & 0.0 & 9 \\
\emph{ibm-employee-performance} & 43897 & 1470 & 33 & 2 & 5 & 25 & 0.0 & 9 \\
\emph{mushroom} & 43922 & 8124 & 22 & 5 & 16 & 0 & 0.0 & 12 \\ \bottomrule
\end{tabular}
\\
\vspace{0.1cm} {\normalfont ID is the OpenML id; obs is the number of entries; feats is the number of features; bins, cats, and nums are the number of binary, categorical, resp. numerical features; \%nans is th percentage of missing values; mostclasses is the greatest number of unique levels of any categorical attribute. The highlighted datasets are the 30 datasets used for full tuning.}
%VA: not sure if this is allowed, but looks better
\end{table*}
